Two-Port Feedback Analysis On Miller-Compensated Amplifiers

In this paper, various Miller-compensated amplifiers are analyzed by using the two-port feedback analysis together with the root-locus diagram. The proposed analysis solves problems of Miller theorem/approximation that fail to predict a pole-splitting and that require an impractical assumption that an initial lower frequency pole before connecting a Miller capacitor in a two-stage amplifier should be associated with the input of the amplifier. Since the proposed analysis sheds light on how the closed-loop poles originate from the open-loop poles in the s-plane, it allows the association of the closed-loop poles with the circuit components and thus provides a design insight for frequency compensation. The circuits analyzed are two-stage Miller-compensated amplifiers with and without a current buffer and a three-stage nested Miller-compensated amplifier.

==> Acknowledgment.tex <==
% use section* for acknowledgment
\section*{Acknowledgment}
The authors would like to thank IC Design Education Center (IDEC), Daejeon, South Korea, for multi project wafer (MPW) and electronic design automation (EDA) support.

==> Appendices_-_bk_0115.tex <==
\appendices
\section{Two-port Feedback Analysis on Miller Compensated Two-stage Operational Amplifier}
\newcounter{mytempeqncnt}
\begin{figure*}[b]
\hrulefill
\vspace*{4pt}
\setcounter{mytempeqncnt}{\value{equation}} 
\setcounter{equation}{21}  
\begin{subequations} \label{ClTF1TF2}
\begin{align} 
H(s)& = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF1}     \\ 
 & = -\frac{g_mR_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o}) + C_c^2]} \label{ClosedTF2} 
\end{align}
\end{subequations}
\begin{subequations} \label{ClTF3TF4}
\begin{align} 
H_{\textrm{direct}}(s)& =  -\frac{(g_m-sC_c)R_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o})]} \qquad \qquad    \label{ClosedTF3}  \\ 
 & = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF4}
\end{align}
\end{subequations}
\setcounter{equation}{\value{mytempeqncnt}}
\end{figure*}
The traditional Miller-compensated two-stage operational amplifier (op-amp) is analyzed using the two-port feedback analysis (TFA)~\cite{Sedra} here. The circuit is shown in Fig.~\ref{FigApp1}(a). The transconductance, lumped resistance, and capacitance at the input $v_{in}$ node (at the output $v_{o}$ node) are modeled as $g_m$, $R_{in}$ ($R_{o}$), $C_{in}$ ($C_{o}$), respectively. Also, $i_{s}$ represents the input signal current to the circuit, and $C_c$ represents a compensating capacitor. The circuit can be considered a feedback amplifier having a shunt-shunt feedback topology as illustrated in Fig.~\ref{FigApp1}(b); the basic amplifier is a unilateral trans-impedance amplifier, and the feedback network is the compensating capacitor that samples the output voltage $v_{o}$, and provides the feedback current $i_{f}$ subtracted from the input signal current $i_{s}$ at the input node. Thus, we apply the rules of the corresponding two-port feedback analysis to find its $A$ circuit, and $\beta$ circuit, giving forward transfer function $a(s)$, and feedback transfer function $\beta(s)$, respectively.

Fig.~\ref{FigApp1}(c) shows the small-signal model of the $A$ circuit with its input current $i_{in}$ including a loading effect of the feedback network, and its associated forward transfer function before ($a(s)$), and after ($a'(s)$) shunting a current source $sC_cv_{in}$ at the output node that reflects the feedforward current through $C_c$, respectively. That signal feedforward transmission through the feedback network, and thus a resulting right-half-plane (RHP) zero, are ignored in the following analysis; however, the analysis including the effect of the RHP zero will be dealt later. 

The forward transfer function $a(s)$ can be easily found by inspection due to its open-loop characteristic, and is given by
\begin{align}
a(s) & \equiv   \frac{v_o(s)}{i_{in}(s)} \nonumber \\ 
& = -\frac{g_mR_{in}R_{o}}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]} \label{eq3} 
\end{align}
where $X\parallel Y = XY/(X+Y)$. From~(\ref{eq3}), $a(s)$ has two left-half-plane (LHP) real poles given by
\begin{subequations} \label{pinandpo}
\begin{align} 
p_{in} & = -\frac{1}{R_{in}(C_{in}+C_c)}  \label{pin}  \\
p_{o} &  = -\frac{1}{R_{o}(C_{o}+C_c)}.    \label{po}
\end{align}
\end{subequations}
Fig.~\ref{FigApp1}(d) shows the small-signal model of the $\beta$ circuit, and its associated feedback transfer function $\beta(s)$ is given by
\begin{align}
\beta(s) \equiv \frac{i_f(s)}{v_{o}(s)} = -sC_c \label{betafunc} 
\end{align}
From~(\ref{betafunc}), $\beta(s)$ has a zero $z_{\beta}$ at the origin (i.e., $z_{\beta} = 0$). 

Combining (\ref{eq3}) and (\ref{betafunc}), the $a(s)\beta(s)$ is expressed as

\begin{align}
 a(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]}. \label{LT1} 
\end{align}

Substituting~(\ref{eq3}), (\ref{LT1}) into the feedback equation~$H(s) = a(s)/(1+a(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H(s) = v_o(s)/i_s(s)$ can be found as~(\ref{ClTF1TF2}) shown at the bottom of the page. The exact closed-loop transfer function $H_{\textrm{direct}}(s)$ is also shown as~(\ref{ClTF3TF4}) obtained by the direct analysis to investigate the validity of the two-port feedback analysis. Comparing~(\ref{ClosedTF1}) with (\ref{ClosedTF4}) shows that the only difference is that $g_m$ has been replaced by ($g_m - sC_c$). This difference stems from the feedforward through $C_c$ that results in a generation of a RHP zero $z_{RHP}= g_m/C_c$ which provides the closed-loop transfer function with a proper sign reversal at DC when plotted in the $s$-plane, and a magnitude-extension of the non-dominant pole by subtracting ${C_c}^2$ from the coefficient of $s^2R_{in}R_o$ in the denominator of (\ref{ClosedTF2}), yielding~(\ref{pndRHP}).\footnote{For this reason, if the effect of the signal feedforward through the feedback network is assumed to be neglected, the denominator of (\ref{ClosedTF2}) should be investigated rather than that of (\ref{ClosedTF3}) to find the poles of the closed-loop transfer function.} That feedforward was assumed to be ignored in the analysis here; (\ref{ClosedTF4}) can be also obtained by the two-port feedback analysis with the forward transfer function $a'(s)$, rather than $a(s)$. Thus, the analysis here is reasonably accurate if $g_m \gg \abs{sC_c}$ at the frequencies of interest.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp2}
\caption{Root-locus diagram for (\ref{LT1}), and the pole-splitting relation.}
\label{FigApp2}
\end{figure}
The poles of the $H(s)$ can be found by drawing the root-locus diagram shown in Fig.~\ref{FigApp2} rather than by directly factoring the denominator of (\ref{ClosedTF2}). It includes the both cases that the $p_{d,init}=p_{in}$ (i.e., $R_{in}(C_{in}+C_c) > R_{o}(C_{o}+C_c)$), and the $p_{d,init}=p_{o}$ (i.e., $R_{o}(C_{o}+C_c) > R_{in}(C_{in}+C_c)$). The resulting diagram shows important facts: 

(1) Regardless of the condition about the $p_{d,init}$ location, the diagram shows the two initial poles must always be splitted as $L_{MID}$ increases; $p_{d,init} \rightarrow 0^-$, $p_{nd,init} \rightarrow -\infty$ as $L_{MID} \rightarrow \infty$; it agrees with~\cite{WHKi}. 

(2) It also predicts that the closed-loop transfer function has only the two real LHP poles since $z_\beta$ at the origin is a zero of $\beta(s)$, and $a(s)$ has no zeros; it can be confirmed by~(\ref{ClosedTF2}).

(3) The locations of the closed-loop dominant ($p_d$), and non-dominant ($p_{nd}$) poles can be found as follows: (\ref{LT1}) can be written in the form  



\addtocounter{equation}{2}
\begin{align*}
 a(s)\beta(s) = \frac{L_{MID}\frac{s}{\abs{p_{d,init}}}}{(1+\frac{s}{\abs{p_{d,init}}})(1+\frac{s}{\abs{p_{nd,init}}})}. 
\end{align*}
Assuming $L_{MID} \gg 1$, the zeros of the characterisitic equation $1 + a(s)\beta(s)$ can be approximately found by solving the following polynomial  
\begin{align}
D(s)  = 1+s\frac{L_{MID}}{\abs{p_{d,init}}} +s^2\frac{1}{\abs{p_{d,init}}\abs{{p_{nd,init}}}}.  \label{LT3} 
\end{align}
If the two roots of $D(s)$ are real and widely spaced (i.e., $\abs{p_{nd}} \gg \abs{p_d}$) , which is typically true, then
\begin{align}
D(s) \simeq 1+s\frac{1}{\abs{p_{d}}} +s^2\frac{1}{\abs{p_{d}}\abs{{p_{nd}}}}.  \label{LT4} 
\end{align}
Equating the coefficient of $s$ in~(\ref{LT3}) and in~(\ref{LT4}) results in 
\begin{align}
\abs{p_d} \simeq \frac{\abs{p_{d,init}}}{L_{MID}}.  \label{pd} 
\end{align}
Similarly, the $p_{nd}$ can be estimated by equating coefficients of $s^2$ in~(\ref{LT3}) and in~(\ref{LT4}), and using~(\ref{pd}).
\begin{align}
\abs{p_{nd}} \simeq L_{MID} \abs{p_{nd,init}}.  \label{pnd} 
\end{align}
Using (\ref{pd}), (\ref{pnd}), we can establish a following simple \textbf{pole-splitting relation}: 
\begin{equation}
  \boxed{L_{MID}  \simeq \frac{p_{d,init}}{p_d}  \simeq \frac{p_{nd}}{p_{nd,init}}}. \label{PoleSplit}
\end{equation}
Using the pole-splitting relation, the locations of the closed-loop poles for any system whose loop-transmission has two LHP real poles and a zero at the origin can be easily obtained. Depending on the condition whether the $p_{d,init} = p_{in}$ or $p_{d,init} = p_{o}$, $L_{MID}$s are differently expressed as 
\begin{equation}
    L_{MID} = 
    \begin{cases}
    \begin{split}
      \frac{g_mR_oC_c}{C_{in}+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{in}     \\
      \frac{g_mR_{in}C_c}{C_o+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{o}   \label{LMID}
    \end{split}
    \end{cases}
\end{equation}
and both cases are graphically illustrated as shown in Fig.~\ref{Fig5}(a), (b), respectively. Substitution of~(\ref{pinandpo}) and (\ref{LMID}) into (\ref{PoleSplit}) gives
\begin{equation}
p_{d}  \simeq -\frac{1}{g_mR_{in}R_oC_c}  \label{pd2} 
\end{equation}
\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)}.    \label{pnd2}
\end{equation}
These poles are the same with those obtained by approximately solving the denominator of~(\ref{ClosedTF2}), and are illustrated in Fig.~\ref{Fig4}. It is worth mentioning that (\ref{pnd2}) is smaller than in the case when a current buffer is connected in series with $C_c$ by a factor of $C_{in} /(C_{in} + C_c)$. This can be confirmed by replacing $g_{mp}$, and $C_{o1}$ in~(\ref{CMCpnd}) with $g_{m}$, and $C_{in}$, respectively. It is due to the absence of loading by $C_c$ at the input side of the op-amp in the latter case because of the current buffer.

(\ref{pd2}), (\ref{pnd2}) are also the poles of the input ($Z_{in}(s)$), and the output ($Z_{o}(s)$) impedance of the circuit because the poles of the circuit does not be affected by an excitation source that does not change its natural structure~\cite{Sedra}. However, the location of the zero is different; $Z_{in}(s)$ is defined as $v_{in}(s)/i_{s}(s)$ in Fig.~\ref{FigApp1}(a), modifying its $A$ circuit to yield a forward transfer function as $v_{in}(s)/i_{in}(s)$ in Fig.~\ref{FigApp1}(c), and its $\beta$ circuit to yield a feedback transfer function as $i_{f}(s)/v_{in}(s) = (v_{o}(s)/v_{in}(s))\beta(s)$ in Fig.~\ref{FigApp1}(c), (d). That implies the feedback path has a pole at $s=p_o$, generating a zero at the same location in $Z_{in}(s)$. Similarly, the $Z_{o}(s)$ can be determined by removing $i_{s}(s)$ at $v_{in}$ node, and shunting an independent test current source $i_{t}(s)$ at $v_o$ node, and analyzing the $v_{o}(s)/i_{t}(s)$ in Fig.~\ref{FigApp1}(a); then, its feedback path has a pole at $s=p_{in}$, generating a zero at the same location in $Z_{o}(s)$. Note that $\beta(s)$ is in the feedback path in both cases, and thus $z_{\beta}$ at the origin is not the zero of $Z_{in}(s)$ and $Z_{o}(s)$.
\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp3}
\caption{A Bode magnitude plot for $L(s)$ when the $p_{d,init}$ is either (a)~$p_{in}$, or (b)~$p_o$.}
\label{FigApp3}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp4}
\caption{Pole-zero diagram with its DC magnitude for (a) $H(s)$, (b) $Z_{in}(s)$, and (c) $Z_{o}(s)$.}
\label{FigApp4}
\end{figure}

The pole-zero diagrams for $A(s)$, $Z_{in}(s)$, and $Z_{o}(s)$ are shown in Fig.~\ref{Fig6}(a), (b), and (c), respectively. Note that in each diagram its DC value is also depicted which can be easily obatined by inspection; thus, its associated Bode plot can be drawn trivially. 

It is worth mentioning that if the system is positive feedback system (i.e., if $-g_m$ in Fig.~\ref{FigApp1}(a) is replaced with $+g_m$), then the root-locus diagram would be drawn with negative locus rules applied; the two intial poles attracts each other, rather than splitted, as $L_{MID}$ increases, and forms complex-conjugate pole-pair when $L_{MID}$ is larger than some finite value at which the two LHP poles coincides. This observation may provide insights to design high $Q$ filters using positive feedback such as the Sallen-Key circuits~\cite{Sallen}.



Fig.~\ref{FigApp1}(c) also shows the $A$ circuit including a loading effect of the feedback network, and its associated forward transfer function $a'(s)$ after adding a current source $sC_cv_{in}$ that reflects the feedforward current thorugh $C_c$, respectively. $a'(s)$ can be found easily by inspection, and is given by
\begin{align}
a'(s)  \equiv  \frac{v'_o(s)}{i_{in}(s)}  = -\frac{g_mR_{in}R_{o}(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}	\label{aprimefunc}	
\end{align}
\noindent where $p_{in}$, $p_{o}$ are expressed as (\ref{pin}), (\ref{po}), respectively, and $z_{RHP} = g_m/C_c$.

(\ref{aprimefunc}) combined with~(\ref{betafunc}) yields the the $a'(s)\beta(s)$ is expressed as
\begin{align}
   a'(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})} \label{aprimebeta} 
\end{align}

Substituting~(\ref{aprimefunc}), (\ref{aprimebeta}) into the the feedback equation~$H'(s) = a'(s)/(1+a'(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H'(s) = v'_o(s)/i_s(s)$ is given by~(\ref{ClosedTF4}) which is exactly the same with~(\ref{ClosedTF3}) obtained by the direct analysis, strictly validating the two-port analysis. 

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp5}
\caption{Root-locus diagram for (\ref{aprimebetaMod}) with negative locus rules applied.}
\label{FigApp5}
\end{figure}


Before the root locus diagram for~(\ref{aprimebeta}) is drawn, a special care must be given \cite{Roberge}; since (\ref{aprimebeta}) does not reflect the sign reversal at $s = 0^+$ associated with the $z_{RHP}$ when plotted in the $s$-plane, it should be slightly modified as 
\begin{align}
   \textrm{Modified} \,\, a'(s)\beta(s) = \frac{-g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}. \label{aprimebetaMod} 
\end{align}
Since (\ref{aprimebetaMod}) has a negative sign at its midband frequency, the system is now considered a positive feedback system. Thus, root locus diagram is drawn with negative locus rules applied is shown in Fig.~\ref{FigApp5}. 

The diagram shows the two initial poles must always be splitted as $L_{MID}$ increases, regardless of the condition about the $p_{d,init}$ location as in the case that the signal feedforward thorugh $C_c$ is ignored. Also, the diagram also predicts that the closed-loop transfer function $H'(s) = v'_o(s)/i_s(s)$ has the two real LHP poles ($p_{d}$, $p_{nd}$), and one zero in RHP ($z_{RHP}$) since the $z_\beta$ at the origin is from $\beta(s)$, and the $z_{RHP}$ stems from $a'(s)$; it can be confirmed by~(\ref{ClosedTF3}).

To determine the closed-loop poles locations, the pole-splitting relation (\ref{PoleSplit}) cannot be blindly applied here, because (\ref{PoleSplit}) has been derived from the loop-transmission that has the two LHP poles and a zero at the origin. However, the resulting pole locations can be described intuitively through nonrigorous terms as follows. $\abs{p_{d,init}},\abs{p_{nd,init}}$ are typically much smaller than $z_{RHP}$ because $z_{RHP}$ is linearly proportinal to $g_m$. Therefore, $z_{RHP}$ has little effect on the loop-transmission magnitudes at the frequencies $\omega = \abs{p_{d,init}}, \abs{p_{nd,init}}$ . Thus, $p_d$, which is located at much lower frequency than $p_{d,init}$, is the same with~(\ref{pd}). However, as $p_{nd,init}$ goes to higher frequency, its magnitude is becoming comparable to that of $z_{RHP}$. This zero increases the loop-transmission magnitude at the high frequency, causing the closed-loop non-dominant pole to be located at a higher frequency than (\ref{pnd}).

Such extension of the non-dominant pole can also be explained using the root-locus diagram shown in Fig.~\ref{FigApp5}. As $L_{MID} \rightarrow \infty$, $p_{nd,init} \rightarrow z_{RHP}^+$, implying $p_{nd}$ can be located at nearer to the $-\infty$ than the case without $z_{RHP}^+$ at the finite $L_{MID}$ applied. It can be verified by factoring the denominator of (\ref{ClosedTF4}), apprixmiately yielding the dominant pole as the same with~(\ref{pd}), and the non-domiant pole as 

\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)-{C_c}^2}   \label{pndRHP}
\end{equation}
whose magnitude is obviously larger than that of~(\ref{pnd2}). 

\begin{figure}[t]
\centering
\includegraphics[width=2.45in]{Figs/FigApp6}
\caption{Skewed differential pair with active current mirror to investigate the locations of zeros.}
\label{FigApp6}
\end{figure}
% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{Zeros for Gain of Skewed Differential Pair}
A skewed differential pair with active current mirror is shown in Fig.~\ref{FigApp6}. We assume that the size of $M_1$ is much larger than that of other devices, and thus a gate-to-drain capacitance of $M_1$ ($C_{gd}$) is included here. The current $i_{\textrm{x}}$ is the drain current of $M_\textrm{x}$, $i_{o1}$ is the amplifier output current, $i_{ff}$ is the feedforward current from $v_{in}$ to $v_{o1}$ through $C_{gd}$, and the arrows indicate their directions. $C_{o1}$, and $C_c$ are the lumped  capacitor at $v_{o1}$ node, and $v_{c}$ node, respectively. 

At zeros of the amplifier gain transfer funcition, $v_{o1} = 0$. Thus, there is no current flow into $C_{o1}$ (i.e., $i_{o1} = 0$.). Then, the locations of the zeros can be obatined by applying KCL at $v_{o1}$ node with $i_{o1} = 0$. For simplicity, we assumed that $g_{m1L} = g_{m1R} \equiv g_{m1}$, and the source node of input-pair is virtual ground (i.e., $i_{1L} = -i_{1R}$). Then, we can write 
\begin{align*}
i_{1L} & = -\frac{g_{m1}v_{in}}{2}   \\
i_{3L} & = -\frac{g_{m1}v_{in}}{2}\frac{g_{m3L}}{g_{m3R}+sC_c} \\
i_{ff} & = sC_{gd}v_{in}.  
\end{align*}
Solving $i_{1L} + i_{3L} + i_{ff} = 0$ with some algebraic manipulations result in the zeros for the amplifier gain are the roots of  
\begin{equation*}
2C_{gd}C_cs^2 + (2g_{m3R}C_{gd}-g_{m1}C_c)s - g_{m1}(g_{m3L}+g_{m3R}) = 0.  \label{zeroroot}
\end{equation*}
Thus, there are two zeros located at LHP ($z_{L}$), and at RHP ($z_{R}$) as given by 
\begin{align}
z_{L,R}  = \frac{g_{m1}}{4C_{gd}}-\frac{g_{m3R}}{2C_{c}} \pm \frac{\sqrt{\Delta}}{4C_cC_{gd}}  \label{z2z3} 
\end{align}
where $\Delta=$
\begin{align*}
g_{m1}^2C_c^2+4g_{m1}g_{m3R}C_cC_{gd}+8g_{m1}g_{m3L}C_cC_{gd}+4g_{m3R}^2C_{gd}^2. 
\end{align*}
If $C_{gd}$ is large so that $g_{m1}/4C_{gd} < g_{m3R}/2C_{c}$, $\abs{z_{L}} > \abs{z_{R}}$. 

==> Appendices_BK0106.tex <==
\appendices
\section{}
\newcounter{mytempeqncnt}
\begin{figure*}[b]
\hrulefill
\vspace*{4pt}
\setcounter{mytempeqncnt}{\value{equation}} 
\setcounter{equation}{6}  
\begin{subequations} \label{ClTF1TF2}
\begin{align} 
H(s)& = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF1}     \\ 
 & = -\frac{g_mR_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o}) + C_c^2]} \label{ClosedTF2} 
\end{align}
\end{subequations}
\begin{subequations} \label{ClTF3TF4}
\begin{align} 
H_{\textrm{direct}}(s)& =  -\frac{(g_m-sC_c)R_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o})]} \label{ClosedTF3}  \\ 
 & = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF4}
\end{align}
\end{subequations}
\setcounter{equation}{\value{mytempeqncnt}}
\end{figure*}
The traditional Miller-compensated two-stage op-amp is analyzed using the two-port feedback analysis (TFA)~\cite{Sedra} here. The circuit is shown in Fig.~\ref{FigApp1}(a). The transconductance, lumped resistance, and capacitance at the input $v_{in}$ node (at the output $v_{o}$ node) are modeled as $g_m$, $R_{in}$ ($R_{o}$), $C_{in}$ ($C_{o}$), respectively. Also, $i_{s}$ represents the input signal current to the circuit, and $C_c$ represents a compensating capacitor. The circuit can be considered a feedback amplifier having a shunt-shunt feedback topology as illustrated in Fig.~\ref{FigApp1}(b); the basic amplifier is a unilateral trans-impedance amplifier, and the feedback network is the compensating capacitor that samples the output voltage $v_{o}$, and provides the feedback current $i_{f}$ subtracted from the input signal current $i_{s}$ at the input node. Thus, we apply the rules of the corresponding two-port feedback analysis to find its $A$ circuit, and $\beta$ circuit, giving forward transfer function $a(s)$, and feedback transfer function $\beta(s)$, respectively.

Fig.~\ref{FigApp1}(c) shows the small-signal model of the $A$ circuit with its input current $i_{in}$ including a loading effect of the feedback network, and its associated forward transfer function before ($a(s)$), and after ($a'(s)$) shunting a current source $sC_cv_{in}$ at the output node that reflects the feedforward current through $C_c$, respectively. That signal feedforward transmission through the feedback network, and thus a resulting right-half-plane (RHP) zero, are ignored in the following analysis; however, the analysis including the effect of the RHP zero will be dealt later. 
\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp1}
\caption{(a) Traditional Miller-compensated two-stage op-amp. (b) Feedback amplifier with a shunt-shunt feedback topology. (c) Small-signal model of the $A$ circuit with the definition of $a(s)$ and $a'(s)$. (d) Small-signal model of the $\beta$ circuit with the definition of $\beta(s)$.}
\label{FigApp1}
\end{figure}
The forward transfer function $a(s)$ can be easily found by inspection due to its open-loop characteristic, and is given by
\begin{align}
a(s) & \equiv   \frac{v_o(s)}{i_{in}(s)} \nonumber \\ 
& =  -(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)}) \nonumber \\ 
& = -\frac{g_mR_{in}R_{o}}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]} \label{eq3} 
\end{align}
where $X\parallel Y = XY/(X+Y)$. From~(\ref{eq3}), $a(s)$ has two left-half-plane (LHP) real poles given by
\begin{subequations} \label{pinandpo}
\begin{align} 
p_{in} & = -\frac{1}{R_{in}(C_{in}+C_c)}  \label{pin}  \\
p_{o} &  = -\frac{1}{R_{o}(C_{o}+C_c)}.    \label{po}
\end{align}
\end{subequations}
Fig.~\ref{FigApp1}(d) shows the small-signal model of the $\beta$ circuit, and its associated feedback transfer function $\beta(s)$ is given by
\begin{align}
\beta(s) \equiv \frac{i_f(s)}{v_{o}(s)} = -sC_c \label{betafunc} 
\end{align}
From~(\ref{betafunc}), $\beta(s)$ has a zero $z_{\beta}$ at the origin (i.e., $z_{\beta} = 0$). 

Combining (\ref{eq3}) and (\ref{betafunc}), the $a(s)\beta(s)$ is expressed as

\begin{align}
 a(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]}. \label{LT1} 
\end{align}

Substituting~(\ref{eq3}), (\ref{LT1}) into the feedback equation~$H(s) = a(s)/(1+a(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H(s) = v_o(s)/i_s(s)$ can be found as~(\ref{ClTF1TF2}) shown at the bottom of the page. The exact closed-loop transfer function $H_{\textrm{direct}}(s)$ is also shown as~(\ref{ClTF3TF4}) obtained by the direct analysis to investigate the validity of the two-port feedback analysis. Comparing~(\ref{ClosedTF1}) with (\ref{ClosedTF4}) shows that the only difference is that $g_m$ has been replaced by ($g_m - sC_c$). This difference stems from the feedforward through $C_c$ that results in a generation of a RHP zero $z_{RHP}= g_m/C_c$ which provides the closed-loop transfer function with a proper sign reversal at DC when plotted in the $s$-plane, and a magnitude-extension of the non-dominant pole by subtracting ${C_c}^2$ from the coefficient of $s^2R_{in}R_o$ in the denominator of (\ref{ClosedTF2}), yielding~(\ref{pndRHP}).\footnote{For this reason, if the effect of the signal feedforward through the feedback network is assumed to be neglected, the denominator of (\ref{ClosedTF2}) should be investigated rather than that of (\ref{ClosedTF3}) to find the poles of the closed-loop transfer function.} That feedforward was assumed to be ignored in the analysis here; (\ref{ClosedTF4}) can be also obtained by the two-port feedback analysis with the forward transfer function $a'(s)$, rather than $a(s)$. Thus, the analysis here is reasonably accurate if $g_m \gg \abs{sC_c}$ at the frequencies of interest.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp2}
\caption{Root-locus diagram for (\ref{LT1}), and the pole-splitting relation.}
\label{FigApp2}
\end{figure}
The poles of the $H(s)$ is found by drawing the root-locus diagram shown in Fig.~\ref{FigApp2} rather than by directly factoring the denominator of (\ref{ClosedTF2}). It includes the both cases that the $p_{d,init}=p_{in}$ (i.e., $R_{in}(C_{in}+C_c) > R_{o}(C_{o}+C_c)$), and the $p_{d,init}=p_{o}$ (i.e., $R_{o}(C_{o}+C_c) > R_{in}(C_{in}+C_c)$). The resulting diagram shows important facts: 

(1) Regardless of the condition about the $p_{d,init}$ location, the diagram shows the two initial poles must always be splitted as $L_{MID}$ increases; $p_{d,init} \rightarrow 0^-$, $p_{nd,init} \rightarrow -\infty$ as $L_{MID} \rightarrow \infty$; it agrees with~\cite{WHKi}. 

(2) It also predicts that the closed-loop transfer function has only the two real LHP poles since the $z_\beta$ at the origin is a phantom zero, and $a(s)$ has no zeros; it can be confirmed by~(\ref{ClosedTF2}).

(3) The locations of the closed-loop dominant ($p_d$), and non-dominant ($p_{nd}$) poles can be found as follows: (\ref{LT1}) can be written in the form  

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp3}
\caption{A Bode magnitude plot for $L(s)$ when the $p_{d,init}$ is either (a)~$p_{in}$, or (b)~$p_o$. Note that $L_{MID}$ is different in each case.}
\label{FigApp3}
\end{figure}

\addtocounter{equation}{2}
\begin{align*}
 a(s)\beta(s) = \frac{L_{MID}\frac{s}{\abs{p_{d,init}}}}{(1+\frac{s}{\abs{p_{d,init}}})(1+\frac{s}{\abs{p_{nd,init}}})}. 
\end{align*}
Assuming $L_{MID} \gg 1$, the zeros of the characterisitic equation $1 + a(s)\beta(s)$ can be approximately found by solving the following polynomial  
\begin{align}
D(s)  = 1+s\frac{L_{MID}}{\abs{p_{d,init}}} +s^2\frac{1}{\abs{p_{d,init}}\abs{{p_{nd,init}}}}.  \label{LT3} 
\end{align}
If the two roots of $D(s)$ are real and widely spaced (i.e., $\abs{p_{nd}} \gg \abs{p_d}$) , which is typically true, then
\begin{align}
D(s) \simeq 1+s\frac{1}{\abs{p_{d}}} +s^2\frac{1}{\abs{p_{d}}\abs{{p_{nd}}}}.  \label{LT4} 
\end{align}
Equating the coefficient of $s$ in~(\ref{LT3}) and in~(\ref{LT4}) results in 
\begin{align}
\abs{p_d} \simeq \frac{\abs{p_{d,init}}}{L_{MID}}.  \label{pd} 
\end{align}
Similarly, the $p_{nd}$ can be estimated by equating coefficients of $s^2$ in~(\ref{LT3}) and in~(\ref{LT4}), and using~(\ref{pd}).
\begin{align}
\abs{p_{nd}} \simeq L_{MID} \abs{p_{nd,init}}.  \label{pnd} 
\end{align}
Using (\ref{pd}), (\ref{pnd}), we can establish a following simple \textbf{pole-splitting relation}: 
\begin{equation}
  \boxed{L_{MID}  \simeq \frac{p_{d,init}}{p_d}  \simeq \frac{p_{nd}}{p_{nd,init}}}. \label{PoleSplit}
\end{equation}
Using the pole-splitting relation, the locations of the closed-loop poles for any system whose loop-transmission has two LHP real poles and a zero at the origin can be easily obtained. Depending on the condition whether the $p_{d,init} = p_{in}$ or $p_{d,init} = p_{o}$, $L_{MID}$s are differently expressed as 
\begin{equation}
    L_{MID} = 
    \begin{cases}
    \begin{split}
      \frac{g_mR_oC_c}{C_{in}+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{in}     \\
      \frac{g_mR_{in}C_c}{C_o+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{o}   \label{LMID}
    \end{split}
    \end{cases}
\end{equation}
and both cases are graphically illustrated as shown in Fig.~\ref{Fig5}(a), (b), respectively. Substitution of~(\ref{pinandpo}) and (\ref{LMID}) into (\ref{PoleSplit}) gives
\begin{equation}
p_{d}  \simeq -\frac{1}{g_mR_{in}R_oC_c}  \label{pd2} 
\end{equation}
\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)}.    \label{pnd2}
\end{equation}
These poles are the same with those obtained by approximately solving the denominator of~(\ref{ClosedTF2}), and are illustrated in Fig.~\ref{Fig4}.

(\ref{pd2}), (\ref{pnd2}) are also the poles of the input ($Z_{in}(s)$), and the output ($Z_{o}(s)$) impedance of the circuit because the poles of the circuit does not be affected by an excitation source that does not change its natural structure~\cite{Sedra}. However, the location of the zero is different; $Z_{in}(s)$ is defined as $v_{in}(s)/i_{s}(s)$ in Fig.~\ref{FigApp1}(a), modifying its $A$ circuit to yield a forward transfer function as $v_{in}(s)/i_{in}(s)$ in Fig.~\ref{FigApp1}(c), and its $\beta$ circuit to yield a feedback transfer function as $i_{f}(s)/v_{in}(s) = (v_{o}(s)/v_{in}(s))\beta(s)$ in Fig.~\ref{FigApp1}(c), (d). That implies the feedback path has a pole at $s=p_o$, generating a zero at the same location in $Z_{in}(s)$. Similarly, the $Z_{o}(s)$ can be determined by removing $i_{s}(s)$ at $v_{in}$ node, and shunting an independent test current source $i_{t}(s)$ at $v_o$ node, and analyzing the $v_{o}(s)/i_{t}(s)$ in Fig.~\ref{FigApp1}(a); then, its feedback path has a pole at $s=p_{in}$, generating a zero at the same location in $Z_{o}(s)$. Note that $\beta(s)$ is in the feedback path in both cases, and thus $z_{\beta}$ at the origin is the phantom zero.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp4}
\caption{Pole-zero diagram with its DC magnitude for (a) $A(s)$, (b) $Z_{in}(s)$, and (c) $Z_{o}(s)$.}
\label{FigApp4}
\end{figure}

The pole-zero diagram for $A(s)$, $Z_{in}(s)$, and $Z_{o}(s)$ is shown in Fig.~\ref{Fig6}(a), (b), and (c), respectively. Note that in each diagram its DC value is also depicted which can be easily obatined by inspection; thus, its associated Bode plot can be drawn trivially. 

It is worth mentioning that if the system is positive feedback system (i.e., if $-g_m$ in Fig.~\ref{FigApp1}(a) is replaced with $+g_m$), then the root-locus diagram would be drawn with negative locus rules applied; the two intial poles attracts each other, rather than splitted, as $L_{MID}$ increases, and forms complex-conjugate pole-pair when $L_{MID}$ is larger than some finite value at which the two LHP poles coincides. This observation may provide insights to design high $Q$ filters using positive feedback such as the Sallen-Key circuits~\cite{Sallen}.

\newcounter{mytempeqncnt2}
\begin{figure*}[b]
\hrulefill
\vspace*{4pt}
\setcounter{mytempeqncnt2}{\value{equation}} 
\setcounter{equation}{19}  
\begin{align}
A(s)& \simeq  \frac{ \frac{-g_mR_1R_2(1 + s\frac{C_c}{g_{mc}})}{[1+sR_1C_1][1+sR_2(C_2+C_c)][1+s\frac{C_c\parallel C_2}{g_{mc}}]}}{1+ \frac{-g_mR_1R_2(1 + s\frac{C_c}{g_{mc}})}{[1+sR_1C_1][1+sR_2(C_2+C_c)][1+s\frac{C_c\parallel C_2}{g_{mc}}]}\frac{-sC_c}{1 + s\frac{C_c}{g_{mc}}}  } \label{aaaaa}    
\end{align}
\setcounter{equation}{\value{mytempeqncnt2}}
\end{figure*}

Fig.~\ref{Fig3}(c) also shows the $A$ circuit including a loading effect of the feedback network, and its associated forward transfer function $a'(s)$ after adding a current source $sC_cv_{in}$ that reflects the feedforward current thorugh $C_c$, respectively. $a'(s)$ can be found easily by inspection, and is given by
\begin{align}
a'(s)  \equiv  \frac{v'_o(s)}{i_{in}(s)}  = -\frac{g_mR_{in}R_{o}(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}	\label{aprimefunc}	
\end{align}
\noindent where $p_{in}$, $p_{o}$ is expressed as (\ref{pin}), (\ref{po}), respectively, and $z_{RHP} = g_m/C_c$.

(\ref{aprimefunc}) combined with~(\ref{betafunc}) yields the the $a'(s)\beta(s)$ is expressed as
\begin{align}
   a'(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})} \label{aprimebeta} 
\end{align}

Substituting~(\ref{aprimefunc}), (\ref{aprimebeta}) into the feedback equation~(\ref{eq2}), and following some algebraic manipulation, the closed-loop transfer function $A'(s) = v'_o(s)/i_s(s)$ is given by~(\ref{ClosedTF4}) which is exactly the same with~(\ref{ClosedTF3}) obtained by the direct analysis, strictly validating the two-port analysis. 




Before the root locus diagram for~(\ref{aprimebeta}) is drawn, a special care must be given \cite{Roberge}; since (\ref{aprimebeta}) does not reflect the DC sign reversal\footnote{Strictly, it is a sign reversal at \[ s= \lim_{s\to0^+}s\] since $L'(s)$ has a zero at the origin.} associated with the $z_{RHP}$ when plotted in the $s$-plane, it should be slightly modified as 
\begin{align}
   \textrm{Modified} \,\, a'(s)\beta(s) = \frac{-g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}. \label{aprimebetaMod} 
\end{align}
Since (\ref{aprimebetaMod}) has a negative sign at its midband frequency, the system is now considered a positive feedback system. Thus, root locus diagram is drawn with negative locus rules applied is shown in Fig.~\ref{FigApp1}. 

The diagram shows the two initial poles must always be splitted as $L_{MID}$ increases, regardless of the condition about the $p_{d,init}$ location as in the case that the signal feedforward thorugh $C_c$ is ignored. Also, the diagram also predicts that the closed-loop transfer function $A'(s) = v'_o(s)/i_s(s)$ has the two real LHP poles ($p_{d}$, $p_{nd}$), and a zero in RHP ($z_{RHP}$) since the $z_\beta$ at the origin is a phantom zero, and the $z_{RHP}$ stems from $a'(s)$; it can be confirmed by~(\ref{ClosedTF3}).

To determine the closed-loop poles locations, the pole-splitting relation (\ref{PoleSplit}) cannot be blindly applied here, because (\ref{PoleSplit}) has been derived from the loop-transmission that has the two LHP poles and a zero at the origin. However, the resulting pole locations can be described intuitively through nonrigorous terms as follows. $\abs{p_{d,init}},\abs{p_{nd,init}}$ are typically much smaller than $z_{RHP}$ because $z_{RHP}$ is linearly proportinal to $g_m$. Therefore, $z_{RHP}$ has little effect on the loop-transmission magnitudes at the frequencies $\omega = \abs{p_{d,init}}, \abs{p_{nd,init}}$ . Thus, $p_d$, which is located at much lower frequency than $p_{d,init}$, is the same with~(\ref{pd}). However, as $p_{nd,init}$ goes to higher frequency, its magnitude is becoming comparable to that of $z_{RHP}$. This zero increases the loop-transmission magnitude at the high frequency, causing the closed-loop non-dominant pole to be located at a higher frequency than (\ref{pnd}).

Such extension of the non-dominant pole can also be explained using the root-locus diagram shown in Fig.~\ref{FigApp1}. As $L_{MID} \rightarrow \infty$, $p_{nd,init} \rightarrow z_{RHP}^+$, implying $p_{nd}$ can be located at nearer to the $-\infty$ than the case without $z_{RHP}^+$ at the finite $L_{MID}$ applied. It can be verified by factoring the denominator of (\ref{ClosedTF4}), apprixmiately yielding the dominant pole as the same with~(\ref{pd}), and the non-domiant pole as 

\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)-{C_c}^2}.   \label{pndRHP}
\end{equation}
whose magnitude is obviously larger than that of~(\ref{pnd2}). 




% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{}
Appendix two text goes here.


==> Appendices_BK0107.tex <==
\appendices
\section{Two-port Feedback Analysis on Miller Compensated Two-stage Operational Amplifier}
\newcounter{mytempeqncnt}
\begin{figure*}[b]
\hrulefill
\vspace*{4pt}
\setcounter{mytempeqncnt}{\value{equation}} 
\setcounter{equation}{21}  
\begin{subequations} \label{ClTF1TF2}
\begin{align} 
H(s)& = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF1}     \\ 
 & = -\frac{g_mR_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o}) + C_c^2]} \label{ClosedTF2} 
\end{align}
\end{subequations}
\begin{subequations} \label{ClTF3TF4}
\begin{align} 
H_{\textrm{direct}}(s)& =  -\frac{(g_m-sC_c)R_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o})]} \label{ClosedTF3}  \\ 
 & = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF4}
\end{align}
\end{subequations}
\setcounter{equation}{\value{mytempeqncnt}}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp1}
\caption{(a) Traditional Miller-compensated two-stage op-amp. (b) Feedback amplifier with a shunt-shunt feedback topology. (c) Small-signal model of the $A$ circuit with the definition of $a(s)$ and $a'(s)$. (d) Small-signal model of the $\beta$ circuit with the definition of $\beta(s)$.}
\label{FigApp1}
\end{figure}
The traditional Miller-compensated two-stage op-amp is analyzed using the two-port feedback analysis (TFA)~\cite{Sedra} here. The circuit is shown in Fig.~\ref{FigApp1}(a). The transconductance, lumped resistance, and capacitance at the input $v_{in}$ node (at the output $v_{o}$ node) are modeled as $g_m$, $R_{in}$ ($R_{o}$), $C_{in}$ ($C_{o}$), respectively. Also, $i_{s}$ represents the input signal current to the circuit, and $C_c$ represents a compensating capacitor. The circuit can be considered a feedback amplifier having a shunt-shunt feedback topology as illustrated in Fig.~\ref{FigApp1}(b); the basic amplifier is a unilateral trans-impedance amplifier, and the feedback network is the compensating capacitor that samples the output voltage $v_{o}$, and provides the feedback current $i_{f}$ subtracted from the input signal current $i_{s}$ at the input node. Thus, we apply the rules of the corresponding two-port feedback analysis to find its $A$ circuit, and $\beta$ circuit, giving forward transfer function $a(s)$, and feedback transfer function $\beta(s)$, respectively.

Fig.~\ref{FigApp1}(c) shows the small-signal model of the $A$ circuit with its input current $i_{in}$ including a loading effect of the feedback network, and its associated forward transfer function before ($a(s)$), and after ($a'(s)$) shunting a current source $sC_cv_{in}$ at the output node that reflects the feedforward current through $C_c$, respectively. That signal feedforward transmission through the feedback network, and thus a resulting right-half-plane (RHP) zero, are ignored in the following analysis; however, the analysis including the effect of the RHP zero will be dealt later. 

The forward transfer function $a(s)$ can be easily found by inspection due to its open-loop characteristic, and is given by
\begin{align}
a(s) & \equiv   \frac{v_o(s)}{i_{in}(s)} \nonumber \\ 
& =  -(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)}) \nonumber \\ 
& = -\frac{g_mR_{in}R_{o}}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]} \label{eq3} 
\end{align}
where $X\parallel Y = XY/(X+Y)$. From~(\ref{eq3}), $a(s)$ has two left-half-plane (LHP) real poles given by
\begin{subequations} \label{pinandpo}
\begin{align} 
p_{in} & = -\frac{1}{R_{in}(C_{in}+C_c)}  \label{pin}  \\
p_{o} &  = -\frac{1}{R_{o}(C_{o}+C_c)}.    \label{po}
\end{align}
\end{subequations}
Fig.~\ref{FigApp1}(d) shows the small-signal model of the $\beta$ circuit, and its associated feedback transfer function $\beta(s)$ is given by
\begin{align}
\beta(s) \equiv \frac{i_f(s)}{v_{o}(s)} = -sC_c \label{betafunc} 
\end{align}
From~(\ref{betafunc}), $\beta(s)$ has a zero $z_{\beta}$ at the origin (i.e., $z_{\beta} = 0$). 

Combining (\ref{eq3}) and (\ref{betafunc}), the $a(s)\beta(s)$ is expressed as

\begin{align}
 a(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]}. \label{LT1} 
\end{align}

Substituting~(\ref{eq3}), (\ref{LT1}) into the feedback equation~$H(s) = a(s)/(1+a(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H(s) = v_o(s)/i_s(s)$ can be found as~(\ref{ClTF1TF2}) shown at the bottom of the page. The exact closed-loop transfer function $H_{\textrm{direct}}(s)$ is also shown as~(\ref{ClTF3TF4}) obtained by the direct analysis to investigate the validity of the two-port feedback analysis. Comparing~(\ref{ClosedTF1}) with (\ref{ClosedTF4}) shows that the only difference is that $g_m$ has been replaced by ($g_m - sC_c$). This difference stems from the feedforward through $C_c$ that results in a generation of a RHP zero $z_{RHP}= g_m/C_c$ which provides the closed-loop transfer function with a proper sign reversal at DC when plotted in the $s$-plane, and a magnitude-extension of the non-dominant pole by subtracting ${C_c}^2$ from the coefficient of $s^2R_{in}R_o$ in the denominator of (\ref{ClosedTF2}), yielding~(\ref{pndRHP}).\footnote{For this reason, if the effect of the signal feedforward through the feedback network is assumed to be neglected, the denominator of (\ref{ClosedTF2}) should be investigated rather than that of (\ref{ClosedTF3}) to find the poles of the closed-loop transfer function.} That feedforward was assumed to be ignored in the analysis here; (\ref{ClosedTF4}) can be also obtained by the two-port feedback analysis with the forward transfer function $a'(s)$, rather than $a(s)$. Thus, the analysis here is reasonably accurate if $g_m \gg \abs{sC_c}$ at the frequencies of interest.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp2}
\caption{Root-locus diagram for (\ref{LT1}), and the pole-splitting relation.}
\label{FigApp2}
\end{figure}
The poles of the $H(s)$ is found by drawing the root-locus diagram shown in Fig.~\ref{FigApp2} rather than by directly factoring the denominator of (\ref{ClosedTF2}). It includes the both cases that the $p_{d,init}=p_{in}$ (i.e., $R_{in}(C_{in}+C_c) > R_{o}(C_{o}+C_c)$), and the $p_{d,init}=p_{o}$ (i.e., $R_{o}(C_{o}+C_c) > R_{in}(C_{in}+C_c)$). The resulting diagram shows important facts: 

(1) Regardless of the condition about the $p_{d,init}$ location, the diagram shows the two initial poles must always be splitted as $L_{MID}$ increases; $p_{d,init} \rightarrow 0^-$, $p_{nd,init} \rightarrow -\infty$ as $L_{MID} \rightarrow \infty$; it agrees with~\cite{WHKi}. 

(2) It also predicts that the closed-loop transfer function has only the two real LHP poles since the $z_\beta$ at the origin is a phantom zero, and $a(s)$ has no zeros; it can be confirmed by~(\ref{ClosedTF2}).

(3) The locations of the closed-loop dominant ($p_d$), and non-dominant ($p_{nd}$) poles can be found as follows: (\ref{LT1}) can be written in the form  

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp3}
\caption{A Bode magnitude plot for $L(s)$ when the $p_{d,init}$ is either (a)~$p_{in}$, or (b)~$p_o$. Note that $L_{MID}$ is different in each case.}
\label{FigApp3}
\end{figure}

\addtocounter{equation}{2}
\begin{align*}
 a(s)\beta(s) = \frac{L_{MID}\frac{s}{\abs{p_{d,init}}}}{(1+\frac{s}{\abs{p_{d,init}}})(1+\frac{s}{\abs{p_{nd,init}}})}. 
\end{align*}
Assuming $L_{MID} \gg 1$, the zeros of the characterisitic equation $1 + a(s)\beta(s)$ can be approximately found by solving the following polynomial  
\begin{align}
D(s)  = 1+s\frac{L_{MID}}{\abs{p_{d,init}}} +s^2\frac{1}{\abs{p_{d,init}}\abs{{p_{nd,init}}}}.  \label{LT3} 
\end{align}
If the two roots of $D(s)$ are real and widely spaced (i.e., $\abs{p_{nd}} \gg \abs{p_d}$) , which is typically true, then
\begin{align}
D(s) \simeq 1+s\frac{1}{\abs{p_{d}}} +s^2\frac{1}{\abs{p_{d}}\abs{{p_{nd}}}}.  \label{LT4} 
\end{align}
Equating the coefficient of $s$ in~(\ref{LT3}) and in~(\ref{LT4}) results in 
\begin{align}
\abs{p_d} \simeq \frac{\abs{p_{d,init}}}{L_{MID}}.  \label{pd} 
\end{align}
Similarly, the $p_{nd}$ can be estimated by equating coefficients of $s^2$ in~(\ref{LT3}) and in~(\ref{LT4}), and using~(\ref{pd}).
\begin{align}
\abs{p_{nd}} \simeq L_{MID} \abs{p_{nd,init}}.  \label{pnd} 
\end{align}
Using (\ref{pd}), (\ref{pnd}), we can establish a following simple \textbf{pole-splitting relation}: 
\begin{equation}
  \boxed{L_{MID}  \simeq \frac{p_{d,init}}{p_d}  \simeq \frac{p_{nd}}{p_{nd,init}}}. \label{PoleSplit}
\end{equation}
Using the pole-splitting relation, the locations of the closed-loop poles for any system whose loop-transmission has two LHP real poles and a zero at the origin can be easily obtained. Depending on the condition whether the $p_{d,init} = p_{in}$ or $p_{d,init} = p_{o}$, $L_{MID}$s are differently expressed as 
\begin{equation}
    L_{MID} = 
    \begin{cases}
    \begin{split}
      \frac{g_mR_oC_c}{C_{in}+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{in}     \\
      \frac{g_mR_{in}C_c}{C_o+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{o}   \label{LMID}
    \end{split}
    \end{cases}
\end{equation}
and both cases are graphically illustrated as shown in Fig.~\ref{Fig5}(a), (b), respectively. Substitution of~(\ref{pinandpo}) and (\ref{LMID}) into (\ref{PoleSplit}) gives
\begin{equation}
p_{d}  \simeq -\frac{1}{g_mR_{in}R_oC_c}  \label{pd2} 
\end{equation}
\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)}.    \label{pnd2}
\end{equation}
These poles are the same with those obtained by approximately solving the denominator of~(\ref{ClosedTF2}), and are illustrated in Fig.~\ref{Fig4}.

(\ref{pd2}), (\ref{pnd2}) are also the poles of the input ($Z_{in}(s)$), and the output ($Z_{o}(s)$) impedance of the circuit because the poles of the circuit does not be affected by an excitation source that does not change its natural structure~\cite{Sedra}. However, the location of the zero is different; $Z_{in}(s)$ is defined as $v_{in}(s)/i_{s}(s)$ in Fig.~\ref{FigApp1}(a), modifying its $A$ circuit to yield a forward transfer function as $v_{in}(s)/i_{in}(s)$ in Fig.~\ref{FigApp1}(c), and its $\beta$ circuit to yield a feedback transfer function as $i_{f}(s)/v_{in}(s) = (v_{o}(s)/v_{in}(s))\beta(s)$ in Fig.~\ref{FigApp1}(c), (d). That implies the feedback path has a pole at $s=p_o$, generating a zero at the same location in $Z_{in}(s)$. Similarly, the $Z_{o}(s)$ can be determined by removing $i_{s}(s)$ at $v_{in}$ node, and shunting an independent test current source $i_{t}(s)$ at $v_o$ node, and analyzing the $v_{o}(s)/i_{t}(s)$ in Fig.~\ref{FigApp1}(a); then, its feedback path has a pole at $s=p_{in}$, generating a zero at the same location in $Z_{o}(s)$. Note that $\beta(s)$ is in the feedback path in both cases, and thus $z_{\beta}$ at the origin is the phantom zero.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp4}
\caption{Pole-zero diagram with its DC magnitude for (a) $H(s)$, (b) $Z_{in}(s)$, and (c) $Z_{o}(s)$.}
\label{FigApp4}
\end{figure}

The pole-zero diagram for $A(s)$, $Z_{in}(s)$, and $Z_{o}(s)$ is shown in Fig.~\ref{Fig6}(a), (b), and (c), respectively. Note that in each diagram its DC value is also depicted which can be easily obatined by inspection; thus, its associated Bode plot can be drawn trivially. 

It is worth mentioning that if the system is positive feedback system (i.e., if $-g_m$ in Fig.~\ref{FigApp1}(a) is replaced with $+g_m$), then the root-locus diagram would be drawn with negative locus rules applied; the two intial poles attracts each other, rather than splitted, as $L_{MID}$ increases, and forms complex-conjugate pole-pair when $L_{MID}$ is larger than some finite value at which the two LHP poles coincides. This observation may provide insights to design high $Q$ filters using positive feedback such as the Sallen-Key circuits~\cite{Sallen}.



Fig.~\ref{Fig3}(c) also shows the $A$ circuit including a loading effect of the feedback network, and its associated forward transfer function $a'(s)$ after adding a current source $sC_cv_{in}$ that reflects the feedforward current thorugh $C_c$, respectively. $a'(s)$ can be found easily by inspection, and is given by
\begin{align}
a'(s)  \equiv  \frac{v'_o(s)}{i_{in}(s)}  = -\frac{g_mR_{in}R_{o}(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}	\label{aprimefunc}	
\end{align}
\noindent where $p_{in}$, $p_{o}$ is expressed as (\ref{pin}), (\ref{po}), respectively, and $z_{RHP} = g_m/C_c$.

(\ref{aprimefunc}) combined with~(\ref{betafunc}) yields the the $a'(s)\beta(s)$ is expressed as
\begin{align}
   a'(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})} \label{aprimebeta} 
\end{align}

Substituting~(\ref{aprimefunc}), (\ref{aprimebeta}) into the the feedback equation~$H'(s) = a'(s)/(1+a'(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H'(s) = v'_o(s)/i_s(s)$ is given by~(\ref{ClosedTF4}) which is exactly the same with~(\ref{ClosedTF3}) obtained by the direct analysis, strictly validating the two-port analysis. 




Before the root locus diagram for~(\ref{aprimebeta}) is drawn, a special care must be given \cite{Roberge}; since (\ref{aprimebeta}) does not reflect the DC sign reversal\footnote{Strictly, it is a sign reversal at \[ s= \lim_{s\to0^+}s\] since $L'(s)$ has a zero at the origin.} associated with the $z_{RHP}$ when plotted in the $s$-plane, it should be slightly modified as 
\begin{align}
   \textrm{Modified} \,\, a'(s)\beta(s) = \frac{-g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}. \label{aprimebetaMod} 
\end{align}
Since (\ref{aprimebetaMod}) has a negative sign at its midband frequency, the system is now considered a positive feedback system. Thus, root locus diagram is drawn with negative locus rules applied is shown in Fig.~\ref{FigApp5}. 

The diagram shows the two initial poles must always be splitted as $L_{MID}$ increases, regardless of the condition about the $p_{d,init}$ location as in the case that the signal feedforward thorugh $C_c$ is ignored. Also, the diagram also predicts that the closed-loop transfer function $A'(s) = v'_o(s)/i_s(s)$ has the two real LHP poles ($p_{d}$, $p_{nd}$), and a zero in RHP ($z_{RHP}$) since the $z_\beta$ at the origin is a phantom zero, and the $z_{RHP}$ stems from $a'(s)$; it can be confirmed by~(\ref{ClosedTF3}).

To determine the closed-loop poles locations, the pole-splitting relation (\ref{PoleSplit}) cannot be blindly applied here, because (\ref{PoleSplit}) has been derived from the loop-transmission that has the two LHP poles and a zero at the origin. However, the resulting pole locations can be described intuitively through nonrigorous terms as follows. $\abs{p_{d,init}},\abs{p_{nd,init}}$ are typically much smaller than $z_{RHP}$ because $z_{RHP}$ is linearly proportinal to $g_m$. Therefore, $z_{RHP}$ has little effect on the loop-transmission magnitudes at the frequencies $\omega = \abs{p_{d,init}}, \abs{p_{nd,init}}$ . Thus, $p_d$, which is located at much lower frequency than $p_{d,init}$, is the same with~(\ref{pd}). However, as $p_{nd,init}$ goes to higher frequency, its magnitude is becoming comparable to that of $z_{RHP}$. This zero increases the loop-transmission magnitude at the high frequency, causing the closed-loop non-dominant pole to be located at a higher frequency than (\ref{pnd}).

Such extension of the non-dominant pole can also be explained using the root-locus diagram shown in Fig.~\ref{FigApp5}. As $L_{MID} \rightarrow \infty$, $p_{nd,init} \rightarrow z_{RHP}^+$, implying $p_{nd}$ can be located at nearer to the $-\infty$ than the case without $z_{RHP}^+$ at the finite $L_{MID}$ applied. It can be verified by factoring the denominator of (\ref{ClosedTF4}), apprixmiately yielding the dominant pole as the same with~(\ref{pd}), and the non-domiant pole as 

\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)-{C_c}^2}.   \label{pndRHP}
\end{equation}
whose magnitude is obviously larger than that of~(\ref{pnd2}). 
\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp5}
\caption{Root-locus diagram for (\ref{aprimebetaMod}) with negative locus rules applied.}
\label{FigApp5}
\end{figure}



% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
%\section{}
%Appendix two text goes here.


==> Appendices_bk_0108.tex <==
\appendices
\section{Two-port Feedback Analysis on Miller Compensated Two-stage Operational Amplifier}
\newcounter{mytempeqncnt}
\begin{figure*}[b]
\hrulefill
\vspace*{4pt}
\setcounter{mytempeqncnt}{\value{equation}} 
\setcounter{equation}{21}  
\begin{subequations} \label{ClTF1TF2}
\begin{align} 
H(s)& = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF1}     \\ 
 & = -\frac{g_mR_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o}) + C_c^2]} \label{ClosedTF2} 
\end{align}
\end{subequations}
\begin{subequations} \label{ClTF3TF4}
\begin{align} 
H_{\textrm{direct}}(s)& =  -\frac{(g_m-sC_c)R_{in}R_{o}}{1 + s[R_{in}C_{in} + R_{o}C_{o} + (g_mR_{in}R_{o} + R_{in} + R_{o})C_c] + s^2R_{in}R_{o}[C_{in}C_{o} + C_c(C_{in}+C_{o})]} \qquad \qquad    \label{ClosedTF3}  \\ 
 & = \frac{-(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})}{1+ (R_{in}\parallel \frac{1}{s(C_{in}+C_c)})(g_m-sC_c)(R_{o}\parallel \frac{1}{s(C_{o}+C_c)})sC_c}  \label{ClosedTF4}
\end{align}
\end{subequations}
\setcounter{equation}{\value{mytempeqncnt}}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp1}
\caption{(a) Traditional Miller-compensated two-stage op-amp. (b) Feedback amplifier with a shunt-shunt feedback topology. (c) Small-signal model of the $A$ circuit with the definition of $a(s)$ and $a'(s)$. (d) Small-signal model of the $\beta$ circuit with the definition of $\beta(s)$.}
\label{FigApp1}
\end{figure}
The traditional Miller-compensated two-stage op-amp is analyzed using the two-port feedback analysis (TFA)~\cite{Sedra} here. The circuit is shown in Fig.~\ref{FigApp1}(a). The transconductance, lumped resistance, and capacitance at the input $v_{in}$ node (at the output $v_{o}$ node) are modeled as $g_m$, $R_{in}$ ($R_{o}$), $C_{in}$ ($C_{o}$), respectively. Also, $i_{s}$ represents the input signal current to the circuit, and $C_c$ represents a compensating capacitor. The circuit can be considered a feedback amplifier having a shunt-shunt feedback topology as illustrated in Fig.~\ref{FigApp1}(b); the basic amplifier is a unilateral trans-impedance amplifier, and the feedback network is the compensating capacitor that samples the output voltage $v_{o}$, and provides the feedback current $i_{f}$ subtracted from the input signal current $i_{s}$ at the input node. Thus, we apply the rules of the corresponding two-port feedback analysis to find its $A$ circuit, and $\beta$ circuit, giving forward transfer function $a(s)$, and feedback transfer function $\beta(s)$, respectively.

Fig.~\ref{FigApp1}(c) shows the small-signal model of the $A$ circuit with its input current $i_{in}$ including a loading effect of the feedback network, and its associated forward transfer function before ($a(s)$), and after ($a'(s)$) shunting a current source $sC_cv_{in}$ at the output node that reflects the feedforward current through $C_c$, respectively. That signal feedforward transmission through the feedback network, and thus a resulting right-half-plane (RHP) zero, are ignored in the following analysis; however, the analysis including the effect of the RHP zero will be dealt later. 

The forward transfer function $a(s)$ can be easily found by inspection due to its open-loop characteristic, and is given by
\begin{align}
a(s) & \equiv   \frac{v_o(s)}{i_{in}(s)} \nonumber \\ 
& =  -(R_{in}\parallel \frac{1}{s(C_{in}+C_c)})g_m(R_{o}\parallel \frac{1}{s(C_{o}+C_c)}) \nonumber \\ 
& = -\frac{g_mR_{in}R_{o}}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]} \label{eq3} 
\end{align}
where $X\parallel Y = XY/(X+Y)$. From~(\ref{eq3}), $a(s)$ has two left-half-plane (LHP) real poles given by
\begin{subequations} \label{pinandpo}
\begin{align} 
p_{in} & = -\frac{1}{R_{in}(C_{in}+C_c)}  \label{pin}  \\
p_{o} &  = -\frac{1}{R_{o}(C_{o}+C_c)}.    \label{po}
\end{align}
\end{subequations}
Fig.~\ref{FigApp1}(d) shows the small-signal model of the $\beta$ circuit, and its associated feedback transfer function $\beta(s)$ is given by
\begin{align}
\beta(s) \equiv \frac{i_f(s)}{v_{o}(s)} = -sC_c \label{betafunc} 
\end{align}
From~(\ref{betafunc}), $\beta(s)$ has a zero $z_{\beta}$ at the origin (i.e., $z_{\beta} = 0$). 

Combining (\ref{eq3}) and (\ref{betafunc}), the $a(s)\beta(s)$ is expressed as

\begin{align}
 a(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs}{[1+sR_{in}(C_{in}+C_c)][1+sR_{o}(C_{o}+C_c)]}. \label{LT1} 
\end{align}

Substituting~(\ref{eq3}), (\ref{LT1}) into the feedback equation~$H(s) = a(s)/(1+a(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H(s) = v_o(s)/i_s(s)$ can be found as~(\ref{ClTF1TF2}) shown at the bottom of the page. The exact closed-loop transfer function $H_{\textrm{direct}}(s)$ is also shown as~(\ref{ClTF3TF4}) obtained by the direct analysis to investigate the validity of the two-port feedback analysis. Comparing~(\ref{ClosedTF1}) with (\ref{ClosedTF4}) shows that the only difference is that $g_m$ has been replaced by ($g_m - sC_c$). This difference stems from the feedforward through $C_c$ that results in a generation of a RHP zero $z_{RHP}= g_m/C_c$ which provides the closed-loop transfer function with a proper sign reversal at DC when plotted in the $s$-plane, and a magnitude-extension of the non-dominant pole by subtracting ${C_c}^2$ from the coefficient of $s^2R_{in}R_o$ in the denominator of (\ref{ClosedTF2}), yielding~(\ref{pndRHP}).\footnote{For this reason, if the effect of the signal feedforward through the feedback network is assumed to be neglected, the denominator of (\ref{ClosedTF2}) should be investigated rather than that of (\ref{ClosedTF3}) to find the poles of the closed-loop transfer function.} That feedforward was assumed to be ignored in the analysis here; (\ref{ClosedTF4}) can be also obtained by the two-port feedback analysis with the forward transfer function $a'(s)$, rather than $a(s)$. Thus, the analysis here is reasonably accurate if $g_m \gg \abs{sC_c}$ at the frequencies of interest.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp2}
\caption{Root-locus diagram for (\ref{LT1}), and the pole-splitting relation.}
\label{FigApp2}
\end{figure}
The poles of the $H(s)$ is found by drawing the root-locus diagram shown in Fig.~\ref{FigApp2} rather than by directly factoring the denominator of (\ref{ClosedTF2}). It includes the both cases that the $p_{d,init}=p_{in}$ (i.e., $R_{in}(C_{in}+C_c) > R_{o}(C_{o}+C_c)$), and the $p_{d,init}=p_{o}$ (i.e., $R_{o}(C_{o}+C_c) > R_{in}(C_{in}+C_c)$). The resulting diagram shows important facts: 

(1) Regardless of the condition about the $p_{d,init}$ location, the diagram shows the two initial poles must always be splitted as $L_{MID}$ increases; $p_{d,init} \rightarrow 0^-$, $p_{nd,init} \rightarrow -\infty$ as $L_{MID} \rightarrow \infty$; it agrees with~\cite{WHKi}. 

(2) It also predicts that the closed-loop transfer function has only the two real LHP poles since the $z_\beta$ at the origin is a phantom zero, and $a(s)$ has no zeros; it can be confirmed by~(\ref{ClosedTF2}).

(3) The locations of the closed-loop dominant ($p_d$), and non-dominant ($p_{nd}$) poles can be found as follows: (\ref{LT1}) can be written in the form  

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp3}
\caption{A Bode magnitude plot for $L(s)$ when the $p_{d,init}$ is either (a)~$p_{in}$, or (b)~$p_o$. Note that $L_{MID}$ is different in each case.}
\label{FigApp3}
\end{figure}

\addtocounter{equation}{2}
\begin{align*}
 a(s)\beta(s) = \frac{L_{MID}\frac{s}{\abs{p_{d,init}}}}{(1+\frac{s}{\abs{p_{d,init}}})(1+\frac{s}{\abs{p_{nd,init}}})}. 
\end{align*}
Assuming $L_{MID} \gg 1$, the zeros of the characterisitic equation $1 + a(s)\beta(s)$ can be approximately found by solving the following polynomial  
\begin{align}
D(s)  = 1+s\frac{L_{MID}}{\abs{p_{d,init}}} +s^2\frac{1}{\abs{p_{d,init}}\abs{{p_{nd,init}}}}.  \label{LT3} 
\end{align}
If the two roots of $D(s)$ are real and widely spaced (i.e., $\abs{p_{nd}} \gg \abs{p_d}$) , which is typically true, then
\begin{align}
D(s) \simeq 1+s\frac{1}{\abs{p_{d}}} +s^2\frac{1}{\abs{p_{d}}\abs{{p_{nd}}}}.  \label{LT4} 
\end{align}
Equating the coefficient of $s$ in~(\ref{LT3}) and in~(\ref{LT4}) results in 
\begin{align}
\abs{p_d} \simeq \frac{\abs{p_{d,init}}}{L_{MID}}.  \label{pd} 
\end{align}
Similarly, the $p_{nd}$ can be estimated by equating coefficients of $s^2$ in~(\ref{LT3}) and in~(\ref{LT4}), and using~(\ref{pd}).
\begin{align}
\abs{p_{nd}} \simeq L_{MID} \abs{p_{nd,init}}.  \label{pnd} 
\end{align}
Using (\ref{pd}), (\ref{pnd}), we can establish a following simple \textbf{pole-splitting relation}: 
\begin{equation}
  \boxed{L_{MID}  \simeq \frac{p_{d,init}}{p_d}  \simeq \frac{p_{nd}}{p_{nd,init}}}. \label{PoleSplit}
\end{equation}
Using the pole-splitting relation, the locations of the closed-loop poles for any system whose loop-transmission has two LHP real poles and a zero at the origin can be easily obtained. Depending on the condition whether the $p_{d,init} = p_{in}$ or $p_{d,init} = p_{o}$, $L_{MID}$s are differently expressed as 
\begin{equation}
    L_{MID} = 
    \begin{cases}
    \begin{split}
      \frac{g_mR_oC_c}{C_{in}+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{in}     \\
      \frac{g_mR_{in}C_c}{C_o+C_c} &  \,\,\,\, \text{if } p_{d,init} = p_{o}   \label{LMID}
    \end{split}
    \end{cases}
\end{equation}
and both cases are graphically illustrated as shown in Fig.~\ref{Fig5}(a), (b), respectively. Substitution of~(\ref{pinandpo}) and (\ref{LMID}) into (\ref{PoleSplit}) gives
\begin{equation}
p_{d}  \simeq -\frac{1}{g_mR_{in}R_oC_c}  \label{pd2} 
\end{equation}
\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)}.    \label{pnd2}
\end{equation}
These poles are the same with those obtained by approximately solving the denominator of~(\ref{ClosedTF2}), and are illustrated in Fig.~\ref{Fig4}.

(\ref{pd2}), (\ref{pnd2}) are also the poles of the input ($Z_{in}(s)$), and the output ($Z_{o}(s)$) impedance of the circuit because the poles of the circuit does not be affected by an excitation source that does not change its natural structure~\cite{Sedra}. However, the location of the zero is different; $Z_{in}(s)$ is defined as $v_{in}(s)/i_{s}(s)$ in Fig.~\ref{FigApp1}(a), modifying its $A$ circuit to yield a forward transfer function as $v_{in}(s)/i_{in}(s)$ in Fig.~\ref{FigApp1}(c), and its $\beta$ circuit to yield a feedback transfer function as $i_{f}(s)/v_{in}(s) = (v_{o}(s)/v_{in}(s))\beta(s)$ in Fig.~\ref{FigApp1}(c), (d). That implies the feedback path has a pole at $s=p_o$, generating a zero at the same location in $Z_{in}(s)$. Similarly, the $Z_{o}(s)$ can be determined by removing $i_{s}(s)$ at $v_{in}$ node, and shunting an independent test current source $i_{t}(s)$ at $v_o$ node, and analyzing the $v_{o}(s)/i_{t}(s)$ in Fig.~\ref{FigApp1}(a); then, its feedback path has a pole at $s=p_{in}$, generating a zero at the same location in $Z_{o}(s)$. Note that $\beta(s)$ is in the feedback path in both cases, and thus $z_{\beta}$ at the origin is the phantom zero.

\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp4}
\caption{Pole-zero diagram with its DC magnitude for (a) $H(s)$, (b) $Z_{in}(s)$, and (c) $Z_{o}(s)$.}
\label{FigApp4}
\end{figure}

The pole-zero diagrams for $A(s)$, $Z_{in}(s)$, and $Z_{o}(s)$ are shown in Fig.~\ref{Fig6}(a), (b), and (c), respectively. Note that in each diagram its DC value is also depicted which can be easily obatined by inspection; thus, its associated Bode plot can be drawn trivially. 

It is worth mentioning that if the system is positive feedback system (i.e., if $-g_m$ in Fig.~\ref{FigApp1}(a) is replaced with $+g_m$), then the root-locus diagram would be drawn with negative locus rules applied; the two intial poles attracts each other, rather than splitted, as $L_{MID}$ increases, and forms complex-conjugate pole-pair when $L_{MID}$ is larger than some finite value at which the two LHP poles coincides. This observation may provide insights to design high $Q$ filters using positive feedback such as the Sallen-Key circuits~\cite{Sallen}.



Fig.~\ref{Fig3}(c) also shows the $A$ circuit including a loading effect of the feedback network, and its associated forward transfer function $a'(s)$ after adding a current source $sC_cv_{in}$ that reflects the feedforward current thorugh $C_c$, respectively. $a'(s)$ can be found easily by inspection, and is given by
\begin{align}
a'(s)  \equiv  \frac{v'_o(s)}{i_{in}(s)}  = -\frac{g_mR_{in}R_{o}(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}	\label{aprimefunc}	
\end{align}
\noindent where $p_{in}$, $p_{o}$ are expressed as (\ref{pin}), (\ref{po}), respectively, and $z_{RHP} = g_m/C_c$.

(\ref{aprimefunc}) combined with~(\ref{betafunc}) yields the the $a'(s)\beta(s)$ is expressed as
\begin{align}
   a'(s)\beta(s) = \frac{g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})} \label{aprimebeta} 
\end{align}

Substituting~(\ref{aprimefunc}), (\ref{aprimebeta}) into the the feedback equation~$H'(s) = a'(s)/(1+a'(s)\beta(s))$, and following some algebraic manipulation, the closed-loop transfer function $H'(s) = v'_o(s)/i_s(s)$ is given by~(\ref{ClosedTF4}) which is exactly the same with~(\ref{ClosedTF3}) obtained by the direct analysis, strictly validating the two-port analysis. 




Before the root locus diagram for~(\ref{aprimebeta}) is drawn, a special care must be given \cite{Roberge}; since (\ref{aprimebeta}) does not reflect the sign reversal at $s = 0^+$ associated with the $z_{RHP}$ when plotted in the $s$-plane, it should be slightly modified as 
\begin{align}
   \textrm{Modified} \,\, a'(s)\beta(s) = \frac{-g_mR_{in}R_{o}C_cs(1-\frac{s}{z_{RHP}})}{(1+\frac{s}{\abs{{p_{in}}}})(1+\frac{s}{\abs{{p_{o}}}})}. \label{aprimebetaMod} 
\end{align}
Since (\ref{aprimebetaMod}) has a negative sign at its midband frequency, the system is now considered a positive feedback system. Thus, root locus diagram is drawn with negative locus rules applied is shown in Fig.~\ref{FigApp5}. 

The diagram shows the two initial poles must always be splitted as $L_{MID}$ increases, regardless of the condition about the $p_{d,init}$ location as in the case that the signal feedforward thorugh $C_c$ is ignored. Also, the diagram also predicts that the closed-loop transfer function $A'(s) = v'_o(s)/i_s(s)$ has the two real LHP poles ($p_{d}$, $p_{nd}$), and a zero in RHP ($z_{RHP}$) since the $z_\beta$ at the origin is a phantom zero, and the $z_{RHP}$ stems from $a'(s)$; it can be confirmed by~(\ref{ClosedTF3}).

To determine the closed-loop poles locations, the pole-splitting relation (\ref{PoleSplit}) cannot be blindly applied here, because (\ref{PoleSplit}) has been derived from the loop-transmission that has the two LHP poles and a zero at the origin. However, the resulting pole locations can be described intuitively through nonrigorous terms as follows. $\abs{p_{d,init}},\abs{p_{nd,init}}$ are typically much smaller than $z_{RHP}$ because $z_{RHP}$ is linearly proportinal to $g_m$. Therefore, $z_{RHP}$ has little effect on the loop-transmission magnitudes at the frequencies $\omega = \abs{p_{d,init}}, \abs{p_{nd,init}}$ . Thus, $p_d$, which is located at much lower frequency than $p_{d,init}$, is the same with~(\ref{pd}). However, as $p_{nd,init}$ goes to higher frequency, its magnitude is becoming comparable to that of $z_{RHP}$. This zero increases the loop-transmission magnitude at the high frequency, causing the closed-loop non-dominant pole to be located at a higher frequency than (\ref{pnd}).

Such extension of the non-dominant pole can also be explained using the root-locus diagram shown in Fig.~\ref{FigApp5}. As $L_{MID} \rightarrow \infty$, $p_{nd,init} \rightarrow z_{RHP}^+$, implying $p_{nd}$ can be located at nearer to the $-\infty$ than the case without $z_{RHP}^+$ at the finite $L_{MID}$ applied. It can be verified by factoring the denominator of (\ref{ClosedTF4}), apprixmiately yielding the dominant pole as the same with~(\ref{pd}), and the non-domiant pole as 

\begin{equation}
p_{nd} \simeq -\frac{g_mC_c}{(C_{in}+C_c)(C_o+C_c)-{C_c}^2}.   \label{pndRHP}
\end{equation}
whose magnitude is obviously larger than that of~(\ref{pnd2}). 
\begin{figure}[t]
\centering
\includegraphics[width=3.45in]{Figs/FigApp5}
\caption{Root-locus diagram for (\ref{aprimebetaMod}) with negative locus rules applied.}
\label{FigApp5}
\end{figure}

% you can choose not to have a title for an appendix
% if you want by leaving the argument blank
\section{Zeros for Gain of PTAT Embedded Amplifier}
The PTAT embedded amplifier with internal cascode devices $M_{2L,R}$ neglected for simplicity is shown in Fig.~\ref{FigApp6}. Since the size of $M_1$ is much larger than that of other devices, a gate-to-drain capacitance of $M_1$ ($C_{gd}$) is included here. The current $i_{\textrm{x}}$ is the drain current of $M_\textrm{x}$, $i_{o1}$ is the amplifier output current, $i_{ff}$ is the feedforward current from $v_{in}$ to $v_{o1}$ through $C_{gd}$, and the arrows indicate their directions. The output capacitor $C_{o1}$ and the equivalent single-ended compensating capacitor $C_c$ are attached at $v_{o1}$, and $v_c$ nodes, respectively. 

At zeros of the amplifier gain transfer funcition, $v_{o1} = 0$. Thus, there is no current flow into $C_{o1}$ (i.e., $i_{o1} = 0$.). Then, the locations of the zeros can be obatined by applying KCL at $v_{o1}$ node with $i_{o1} = 0$. Assuming an infinite output resistance of the tail current source and $g_{m1L} = g_{m1R} \equiv g_{m1}$ for simplicity, we can write 
\begin{align*}
i_{1L} & = -i_{1R} = -\frac{g_{m1L}g_{m1R}v_{in}}{g_{m1L}+g_{m1R}}   \\
i_{3L} & = -i_{1R}\frac{g_{m3L}}{g_{m3R}+sC_c} = -\frac{g_{m1L}g_{m1R}g_{m3L}v_{in}}{(g_{m1L}+g_{m1R})(g_{m3R}+sC_c)}  \\
i_{ff} & = sC_{gd}v_{in}.  
\end{align*}
Solving $i_{1L} + i_{3L} + i_{ff} = 0$ with some algebraic manipulations result in the zeros of the amplifier are the roots of  
\begin{equation*}
2C_{gd}C_cs^2 + (2C_{gd}g_{m3R}-C_cg_{m1})s - g_{m1}(g_{m3L}+g_{m3R}) = 0.  \label{zeroroot}
\end{equation*}
Thus, there are two zeros located at RHP ($z_2$), and at LHP ($z_3$) as given by 
\begin{align}
z_{2,3}  = \frac{g_{m1}}{4C_{gd}}-\frac{g_{m3R}}{2C_{c}} \pm \frac{\sqrt{\Delta}}{4C_cC_{gd}}  \label{z22} 
\end{align}
where $\Delta=$
\begin{align*}
C_c^2g_{m1}^2+4C_cC_{gd}g_{m1}g_{m3R}+8C_cC_{gd}g_{m1}g_{m3L}+4C_{gd}^2g_{m3R}^2. 
\end{align*}
When $g_{m1}/4C_{gd} < g_{m3R}/2C_{c}$ that is the case in the proposed BGR, $\abs{z_3} > \abs{z_2}$ as shown in Fig.~\ref{Fig7}(a).


\begin{figure}[t]
\centering
\includegraphics[width=2.45in]{Figs/FigApp6}
\caption{Simplified PTAT embedded amplifier to investigate zero locations.}
\label{FigApp6}
\end{figure}









==> Bibliography.tex <==
\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}

==> Conclusion.tex <==
\section{Conclusion}
The conclusion goes here.

==> Section1_-_bk0110.tex <==
\section{Introduction}

\IEEEPARstart{V}{oltage} reference provides stable DC output voltage that is necessary for almost all electronic systems. Recently, CMOS-only voltage references with ultra-low-power~(ULP) operation~\cite{Vita, Magnelli} have been proposed. However, they are intrinsically vulnarable to process variation because CMOS-only voltage references use a threshold voltage of a MOSFET as a complementary-to-absolute-temperature (CTAT) voltage source. 

On the contrary, a Bandgap reference (BGR) uses the base-emitter voltage ($V_{BE}$) of BJT as the CTAT voltage source, and thus is less affected by process variation. However, many BJTs to generate a proportional-to-absolute-temperature (PTAT) voltage ($V_{PTAT}$) causes BGR to occupy large area, and consume large power. For example, a conventional BGR as shown in Fig.~\ref{Fig1_mod}(a) has two BJT branches whose currents are controlled by the size ratio ($1:8$) of BJTs and a large resistor ($R_1 = 540k\Omega$) to set a bias current of BJT ($I_B$) about 100nA at room temperature. Then, a large $R_{2R}$ of about $6M\Omega$ is needed to generate an output voltage of 1.2V. Moreover, a replica resistor $R_{2L}$ is also needed to minimize current mismatch in the two BJT branches that will incur inaccurate $V_{PTAT}$. Hence, the conventional BGR structure with two BJT branches occupies quite a large area of ($R_1+R_{2R}+R_{2L}+$9BJTs) in addition to the large MOFSETs used in the current-mirror ($M_{PL,R}$) to minimize mismatch.

To mitigate these problems, we previously proposed a BGR that has single BJT branch as shown in Fig.~\ref{Fig1_mod}(b)~\cite{Myungjun2}. As in the case of conventional BGR, CTAT voltage is provided by the $V_{BE}$ of the unit BJT. However, $V_{PTAT}$ is provided by an amplifier which has offset voltage~\cite{Osaki}. To achieve 1.2V output using 100nA of $I_B$, while minimizing temperature coefficient, $R_1$ and $R_2$ can set to around $1.6M\Omega$ and $3.5M\Omega$, respectively. As can be seen, the proposed BGR has fewer resistors, BJT compared to that of the conventional BJR and can be more compact. Moreover, the BJT current consumption (which takes significant portion of the overall power) is also halved.

In this paper, more detailed analysis than~\cite{Myungjun2} on the single BJT BGR is carried out. Espeically, the analysis on frequency compensation is highly extended by using two-port feedback analysis with root-locus diagram, that finally give us the design guideline to obtain the optimum stability and power performance. Also, a start-up issue is added. 

This paper is organized as follows. In Section~II, detailed analysis for the proposed single BJT branch BGR is carried out. In Section~III, experimental results are presented. Section~IV concludes the paper.

==> Table_Backup.tex <==
\begin{table*}[!t]
\setlength{\tabcolsep}{0.1pt}
\renewcommand{\arraystretch}{2.0}
\caption{Comparison with State-Of-The-Arts Cap-less LDOs}
\label{Table2}
\centering
\begin{tabular}{c||c|c|c|c|c|c|c}
\hline
   & \makecell{\cite{Milliken} \\ TCAS-I 2007}   &    \makecell{\cite{Bu} \\ TPE 2018}   &  \makecell{[1] \\ ISSCC 2018}  & \makecell{[2] \\ISSCC 2018}  &  \makecell{[3] \\ ISSSC 2020} & \makecell{[4] \\ ISSCC 2020} & \makecell{\textbf{This Work} } \\ 
\hline
Tech. (nm) & 350 & 130	 & 65 & 28 & 28 & 40 & \textbf{180}   \\ \hline 
Type     & Analog &  Analog	 & Digital & AA-Digital & Digital & Analog & \textbf{Analog} \\ \hline
$V_{DD}$ (V)   & 3 $\sim$ 4.2 & 1 $\sim$ 1.4  &  0.6 $\sim$ 1.2 & 0.4 & 0.5 $\sim$ 1 & 0.4 $\sim$ 1.2  &  \textbf{0.5 $\sim$ 1.8} 	\\\hline
$V_O$ (V) 	&  2.8 &	 0.8 &	0.4 $\sim$ 1.1 & 0.35 & 0.45 $\sim$ 0.95	 & 0.2 $\sim$ 1.18   & \textbf{0.47}  \\\hline
On-chip $C_o$ (pF) 	& 100  & 	0 & 40	& 0 &	0  & 90 & \textbf{0}  \\\hline
Total Area (mm$^2$)  & 0.12   & 0.008 & 0.0374 & 0.0055  &  0.049 & 0.191  & \textbf{0.0035}			\\\hline
$I_Q$ ($\mu$A)    & 65 &  112  & 100 $\sim$ 1,070	  &	0.43  &	7.7 $\sim$ 241 & 4.4 $\sim$ 1,280   &  \textbf{\makecell{22.25 @ 0.5 $\boldsymbol{V_{DD}}$,\\ 35.7 @ 1.8 $\boldsymbol{V_{DD}}$}}  	\\ \hline
$I_{L,MIN}$ (mA)  & 0  &  0.12  & 10 @ 1 $V_{DD}$	 &	1 @ 0.4 $V_{DD}$  &	20 @ 0.9 $V_{DD}$  & \makecell{0.21 @ 0.4 $V_{DD}$,\\ 2 @ 1 $V_{DD}$} &  \textbf{0 @ All $\boldsymbol{V_{DD}}$  }  	\\ \hline
$I_{L,MAX}$ (mA)   & 50 & 25  &	100 & 16  & \makecell{ 160 @ 0.5 $V_{DD}$, \\ 480 @ 1 $V_{DD}$} & \makecell{ 1.25 @ 0.4 $V_{DD}$, \\ 202 @ 1 $V_{DD}$} & \textbf{\makecell{ 2 @ 0.5 $\boldsymbol{V_{DD}}$, \\ 200 @ 1.8 $\boldsymbol{V_{DD}}$}}			  \\\hline
$C_L$ (pF)  & 0 $\sim$ 100 & 0 $\sim$ 25 & N/A & N/A  &  N/A & N/A  & \textbf{0 $\sim$ 50}			\\\hline
 PSR (dB) & \makecell{$-$57 @ 1 kHz \\ (Dropout = 0.2V)} & \makecell{$-$64 @ 1 kHz, \\ $-$57 @ 1 MHz \\   (Dropout = 50mV)} & \makecell{$-$38 @ 10 kHz \\ (Dropout = 0.2V)}    & \makecell{$-$25 @ 100 Hz, \\ $-$1 @ 100 kHz \\   (Dropout = 50mV)}  & N/A &  \makecell{$-$35 @ 1 kHz, \\ $-$32 @ 100 kHz \\   (Dropout = 0.1V)}  & \textbf{\makecell{$-$62 @ 100 Hz, \\ $-$45 @ 100 kHz \\ (Dropout = 30mV)}}	   \\\hline
\makecell{Load Regulation \\ (mV/A)} & \makecell{840 \\ ($I_L$ = 0$\sim$50mA) } & \makecell{173 \\ ($I_L$ = 0.1$\sim$25mA) }    & \makecell{*540 \\ ($I_L$ = 20$\sim$70mA) } &\makecell{510 \\ ($I_L$ = 1$\sim$16mA) } & \makecell{*47 \\ ($I_L$ = 20$\sim$450mA) } & \makecell{*40 \\ ($I_L$ = 2$\sim$202mA) } & \textbf{\makecell{9.5 \\  ($\boldsymbol{I_L}$ = 0$\sim$200mA) }} 	\\\hline
\makecell{Line Regulation \\ (mV/V)}   &  35 &  2.25& *108 & 2.32 & N/A & N/A & \textbf{0.346}            \\\hline
\makecell{ Current Density  \\ (A/mm$^2$)}	&  0.42 &  3.1 & 2.7  &  2.9  & 9.8 & 2.1 & \textbf{57.1}							   \\\hline
FoM$_{\textrm{T}}$ (fs)	& \makecell{81.3 @ 3 $V_{DD}$  \\  ($T_{edge}$ = 1 $\mu$s) }    & \makecell{900 @ 1 $V_{DD}$  \\  ($T_{edge}$ = 0.3 ns) }	& \makecell{1,380 @ 1 $V_{DD}$ \\  ($T_{edge}$ = 800 ns) }   & \makecell{5.1 \\  ($T_{edge}$ = 3 ns) }  &  \makecell{0.41 @ 0.9 $V_{DD}$  \\  ($T_{edge}$ = 2 ns) } 	 & \makecell{28,600 @ 0.4 $V_{DD}$, \\ 55 @ 1 $V_{DD}$ \\ ($T_{edge}$ = 10 ns)  }	 &	\textbf{\makecell{**604 @ 0.5 $\boldsymbol{V_{DD}}$ \\($\boldsymbol{T_{edge}}$ = 100 ns),  \\ **0.27 @ 1.8 $\boldsymbol{V_{DD}}$ \\ ($\boldsymbol{T_{edge}}$ = 300 ns) }}							   \\ \hline
1\% $T_s$ (ns)  & $\leq$ 15,000   & $<$ 190 & 1,240  & 410,000  & 6,000 &  500 &	 \textbf{$\boldsymbol{\leq}$ 862}		      \\\hline
Ripple (m$V_{pp}$)  & 0 &  0 & 120  & *14  & *40	 &  0 &	 \textbf{0}		      \\\hline

\makecell{Output Noise Density\\ ($\mu$V/$\sqrt{Hz}$)} &  0.72 @ 10 kHz  &  N/A & N/A  &  N/A & N/A  & N/A &	 \textbf{\makecell{1.78 @ 100 Hz \\ 0.084 @ 100 kHz}} 		      \\\hline
\end{tabular}
\end{table*}
